Cut and conjugate points of the exponential map, with applications

The goal of this thesis is to study the singularities of the exponential map of Riemannian and Finsler manifolds (a concept related to caustics and catastrophes), and the object known as the cut locus (aka ridge, medial axis or skeleton), to improve existing results about its structure, to look at it in new ways, and to derive applications to the Ambrose conjecture and the Hamilton-Jacobi equations.

==> PreviousKnowledge.tex <==
\chapter{Introduction to the exponential map and the cut locus}

\section{Riemannian and Finsler metrics}
blah

\section{The exponential map and its singularities}
blah

\section{The cut locus}
blah

\section{Hamilton-Jacobi BVPs (boundary value problems)}
blah


